Functional Pearl: Witness Me -- Constructive Arguments Must Be Guided with Concrete Witness

Beloved Curry--Howard correspondence tells that types are intuitionistic propositions, and in constructive math, a proof of proposition can be seen as some kind of a construction, or witness, conveying the information of the proposition. We demonstrate how useful this point of view is as the guiding principle for developing dependently-typed programs.

==> acmart-preload-hook.tex <==
\usepackage[\xcoloropt]{xcolor}


==> switches.tex <==
\RequirePackage{etoolbox}
\newbool{arxiv}
\booltrue{arxiv}
\newbool{arxiv-cached}
\booltrue{arxiv-cached}
\ifbool{arxiv-cached}{\booltrue{arxiv}}{}
\newbool{final}
% \booltrue{final}
\newbool{realname}
\ifbool{arxiv}{%
  \booltrue{realname}%
  \def\xcoloropt{prologue}
}{%
  \ifbool{final}{\booltrue{realname}}{}
  \def\xcoloropt{gray,prologue}
}
\newbool{maingo}
\ifbool{arxiv}{\booltrue{maingo}}{}
\ifbool{final}{\booltrue{maingo}}{}


